Revisiting Hidden Representations in Transfer Learning for Medical Imaging

While a key component to the success of deep learning is the availability of massive amounts of training data, medical image datasets are often limited in diversity and size. Transfer learning has the potential to bridge the gap between related yet different domains. For medical applications, however, it remains unclear whether it is more beneficial to pre-train on natural or medical images. We aim to shed light on this problem by comparing initialization on ImageNet and RadImageNet on seven medical classification tasks. Our work includes a replication study, which yields results contrary to previously published findings. In our experiments, ResNet50 models pre-trained on ImageNet tend to outperform those trained on RadImageNet. To gain further insights, we investigate the learned representations using Canonical Correlation Analysis (CCA) and compare the predictions of the different models. Our results indicate that, contrary to intuition, ImageNet and RadImageNet may converge to distinct intermediate representations, which appear to diverge further during fine-tuning. Despite these distinct representations, the predictions of the models remain similar. Our findings show that the similarity between networks before and after fine-tuning does not correlate with performance gains, suggesting that the advantages of transfer learning might not solely originate from the reuse of features in the early layers of a convolutional neural network.

==> sec6_discussion.tex <==
In our experiments \imagenet{} generally outperformed \radimagenet{} on medical target datasets, in contrast to the earlier results reported in \cite{mei2022radimagenet}. However, this highlights the sensitivity of source dataset transfer performance to the model architecture and hyperparameters, rather than the inherent superiority of one source dataset over the other. While our study did not comprehensively analyze this sensitivity, interested readers can refer to related studies, such as \cite{raghu2019transfusion} and \cite{wen2021rethinking}, which offer valuable insights into the impact of model architecture and hyperparameters on transfer performance.

%% added by Amelia
Contrary to our preconceptions about transfer learning, our analysis with CCA found that the models converged to distinct intermediate representations and that these representations are even more dissimilar after fine-tuning on the same target dataset. Despite distinct intermediate representations, model predictions on an instance level exhibit a significant degree of similarity. This extends \cite{mania2019model} findings which showed that \imagenet{} models are similar in their predictions even with different architectures. We extend upon the findings of \cite{raghu2019transfusion}, who demonstrated limited feature reuse in the lowest two layers of a CNN. We discover that even the features in the first two layers are not reused to the same extent as previously believed.

While our results are similar across seven different target datasets, these tasks are not fully representative of the medical imaging field as a whole. Researchers have hypothesized that for 3D target tasks such as CT or MRI, 3D pre-training might be a better alternative to 2D pre-training \citep{wong2018building,brandt2021cats}, and studies have shown that incorporating information from the third dimension might be beneficial for performance \citep{yang2021reinventing,taleb20203d}. However, \radimagenet{} only has 2D images, even though some of the original images are 3D. From our results, we are unable to conclude that \imagenet{} weights are generally more suitable for medical target tasks. 

Another limitation is in only using AUC as the metric for evaluating performance. Although this is a commonly used metric for classification tasks in medical imaging, there might be nuances across applications where it could be important to consider alternative metrics, such as calibration \citep{reinke2021common}.

Our results suggest that the implications of using \imagenet{} in medical image classification go beyond performance alone. In particular, there might be an issue with the memorization of spurious patterns in the data. This can potentially have consequences with respect to algorithmic bias and fairness. For example, see \cite{gichoya2022ai} where \imagenet{} pre-trained networks memorize patient race. Memorization also makes a network more vulnerable to adversarial attacks \citep{bortsova2021adversarial}. It would be interesting to further explore these properties in future research. 

While \radimagenet{}'s comparable size to \imagenet{} allowed for a unique opportunity to compare natural and medical source datasets, it is important to note that the two datasets have significant differences beyond their domains. For instance, \radimagenet{} has differences in color, number of classes, and diversity in data due to its limited number of patients. To further explore the impact of these differences in greater detail, future research could consider including Ecoset \citep{mehrer2021ecologically}, a natural image dataset with 565 basic-level categories selected to better reflect the human perceptual and cognitive experience.
